Balancing Act: Distribution-Guided Debiasing in Diffusion Models

Diffusion Models (DMs) have emerged as powerful generative models with unprecedented image generation capability. These models are widely used for data augmentation and creative applications. However, DMs reflect the biases present in the training datasets. This is especially concerning in the context of faces, where the DM prefers one demographic subgroup vs others (eg. female vs male). In this work, we present a method for debiasing DMs without relying on additional data or model retraining. Specifically, we propose Distribution Guidance, which enforces the generated images to follow the prescribed attribute distribution. To realize this, we build on the key insight that the latent features of denoising UNet hold rich demographic semantics, and the same can be leveraged to guide debiased generation. We train Attribute Distribution Predictor (ADP) - a small mlp that maps the latent features to the distribution of attributes. ADP is trained with pseudo labels generated from existing attribute classifiers. The proposed Distribution Guidance with ADP enables us to do fair generation. Our method reduces bias across single/multiple attributes and outperforms the baseline by a significant margin for unconditional and text-conditional diffusion models. Further, we present a downstream task of training a fair attribute classifier by rebalancing the training set with our generated data.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}



==> sec/4_experiments.tex <==
\section{Experiments}
\label{sec:exp}
\vspace{-2mm}
In this section, we first discuss the evaluation metrics, followed by the implementation details. We take face datasets as the subject of study, as they are subject to very high demographic biases. We compare our method with other inference time debiasing approaches for both single-attribute and multi-attribute debiasing. Further, we present detailed ablations to validate design choices. Finally, we show the generalization of our debiasing approach on large text-to-image generation model Stable Diffusion~\cite{ldm}. 

\subsection{Evaluation Metrics}
\label{subsec:metrics} 
\vspace{-2mm}
A \textit{fair} generative model is evaluated on two grounds: image quality and fairness.
Therefore, we begin by discussing the metrics we use to measure these two attributes of the generated images.

\noindent \textbf{Fairness}. The primary goal of this paper is to generate images based on the reference distribution $\mathbf{p_{ref}^a}$. We follow Choi et al. ~\cite{choi2020fair} to define the \textbf{Fairness Discrepancy} (FD) metric. Given an attribute $\mathbf{a}$, we assume access to a high-accuracy classifier for $\mathbf{a}$ (denoted as $\mathcal{C}_a$), and using the predictions from the latter, we compute the following~\cite{choi2020fair, teo2023fair}:

$$|\bar{p} - \mathbb{E}_{\mathbf{x} \sim p_\theta(\mathbf{x})}(\mathbf{y})|_2$$
where $\mathbf{y}$ is the softmax output of the classifier $\mathcal{C}_a(\mathbf{x})$, $\bar{p}$ is a uniform vector of the same dimension as $\mathbf{y}$, $p_\theta$ is the distribution of the generated images. The lower the FD score, the closer the distribution of the attribute values is to the uniform distribution -- i.e., the generated images are fairer with respect to attribute $\mathbf{a}$.

\noindent \textbf{Image Quality}. To measure the quality of generation, we follow the standard Fréchet Inception Distance (FID)~\cite{heusel2017gans}. We compute this metric with the help of an attribute-wise balanced dataset sampled from the original training data. 
% by obtaining the distance between the generated distribution $p_\theta$ and a reference distribution $q_{ref}$, which we estimate by sampling all sub-groups of different attributes equally from the original training set. The lower the value of FID, the better the approximation to $q_{ref}$. 


\subsection{Implementation Details}
\label{subsec:implementation}
\vspace{-2mm}
\textbf{Training h-space classifiers.} We start with creating a paired dataset $\mathcal{D}^h_{clf}$ of h-vector and attribute labels. Specifically, we take a subset $\mathcal{D}$ of the CelebA-HQ~\cite{pro-gan} dataset and obtain attribute labels for the images using the pretrained attribute classifier $\mathcal{C}_a$. Next, we embed image $\mathbf{I^i} \in \mathbf{D}$ to obtain the corresponding h-space representation $\mathbf{\mathcal{H}^i} = \{\mathbf{h^i_t}\}^{t=T}_{t=0}$ using DDIM~\cite{ddim} inversion. This yields a labelled dataset $\mathcal{D}^h_{clf}$ with pairs $(\mathcal{H}^i, \mathbf{y^i})$, where $\mathbf{y^i} = \mathcal{C}_a(I^i)$ is the predicted attribute label for image $\mathbf{I^i}$ (\eg \textit{male / female}). Next, we train \textit{h-space} attribute classifiers $\mathcal{C}^h_a(\mathbf{h_t}, t)$ as a \textit{linear} head over $\mathbf{h_t}$ and conditioned on time $t$ (ignored sample index $i$ for brevity). These obtained classifiers generate high-accuracy attribute predictions, as shown in Fig.~\ref{fig:h-space-clf-evals}. Further details about the dataset and classifiers are provided in a supplementary document. 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/cvpr24-debdiff-quals-fig7-balancing.pdf} 
    \vspace{-6mm}
    \caption{\textbf{Balancing generated data across \textit{gender} and \textit{eyeglass} attributes with various guidance strategies.} Minority group \textcolor{Goldenrod}{$male$} and \textcolor{Goldenrod}{$eyeglasses$} are marked. Image-space \textbf{Universal Guidance} and \textbf{Sample Guidance} results generate imbalanced and poor-quality images. For \textit{gender}, Sample Guidance is able to generate only a few \textit{males} while maintaining quality. The proposed \textbf{Distribution Guidance} balances (close to the ratio of $0.50:0.50$) both the attributes and generates high-quality images.}
    \label{fig:single-debias}
\end{figure*}

\noindent 
\textbf{Distribution guidance.} To perform distribution guidance, we realize the distribution prediction function, \textbf{ADP} with \textit{h-space} classifiers $\mathcal{C}^h_a$. Specifically for a generating batch $\mathbf{x_t^{[1:N]}}$, we obtain the corresponding $h-space$ representation $\mathbf{h_t^{[1:N]}}$ and obtain a set of attribute predictions $\mathbf{\hat{y}^{[1:N]}_t}$ from classifiers $\mathcal{C}^h_a$. Finally, we add all the softmax values for all the $N$ images in the batch for each class to obtain the estimate of $\mathbf{p^a_{\theta}}$. We use \textit{Chi-square} distance as the loss $\mathcal{L}$ with the reference distribution $\mathbf{p^a_{ref}}$. 


\noindent \textbf{Diffusion Model Architecture.} We evaluated our proposed debiasing method for fair generation from two state-of-the-art pretrained DMs: a) an unconditional DM, P2 ~\cite{choi2022perception}, trained on CelebA-HQ dataset, and b) a text conditional DM StableDiffusion v1.5 ~\cite{ldm} trained on the LAION~\cite{schuhmann2022laion} dataset. Both these models have exceptional image generation quality; however, they have significant bias concerning the sensitive face attributes, as shown in the following subsections. 

\subsection{Evaluation and Comparisons.}
\vspace{-2mm}
We compare our proposed method against two techniques for guidance-based generations for DMs and a state-of-the-art sampling-based technique for debiasing generative models, MagNet~\cite{humayun2021magnet}.

\noindent \textbf{Sample guidance.} We use classifier guidance as explained in Sec.~\ref{subsec:clf_guide} in the \textit{h-space} using the trained \textit{h-space} attribute classifiers $\mathcal{C}_a^h$. Such guidance requires presetting an attribute state for each generating image and pushing the trajectory to change the attribute state. 

\noindent \textbf{Universal guidance}~\cite{bansal2023universal} performs guidance in the image space but uses pretrained classifiers trained on the clean image. This resolves the additional requirement of training image classifiers on noisy images. The key idea is to use the DDIM scheduler and predict the approximation of $\mathbf{\hat{x_0}}$ from noise image $\mathbf{x_t}$, and pass it through pretrained image classifier $\mathcal{C}_A$. However, this process has two shortcomings. Firstly, it is slow as we have to backpropagate the gradients from the image classifier. Experimentally, we found the \textit{h-space} guidance to be $7$ times faster than the image guidance. Secondly, it performs poorly at the early stage due to an inaccurate approximation of $\mathbf{x_0}$. We used the same training set of $|\mathcal{D}_{clf}| = 2K$ to train the \textit{h-space} and image space attribute classifiers for a fair comparison.     

\begin{table}[]
\vspace{-6mm} 
\caption{Evaluation of \textit{balanced} generation for single attribute}
\vspace{-2mm}
\begin{adjustbox}{width=0.45\textwidth,center}
\begin{tabular}{@{}l|cc|cc|cc@{}}
\toprule
                            & \multicolumn{2}{c|}{Gender}                                                      & \multicolumn{2}{c|}{Race}                                                        & \multicolumn{2}{c}{Eyeglasses}                                                   \\ \midrule
\multicolumn{1}{c|}{Metric} & \multicolumn{1}{c|}{FD}    & \begin{tabular}[c]{@{}c@{}}FID\\ \end{tabular} & \multicolumn{1}{c|}{FD}    & \begin{tabular}[c]{@{}c@{}}FID\\ \end{tabular} & \multicolumn{1}{c|}{FD}    & \begin{tabular}[c]{@{}c@{}}FID\\ \end{tabular} \\ \midrule
Random Sampling             & \multicolumn{1}{c|}{0.178} & 54.59                                               & \multicolumn{1}{c|}{0.334} & 60.01                                               & \multicolumn{1}{c|}{0.251} & 75.21                                               \\
Universal Guidance ~\cite{bansal2023universal}         & \multicolumn{1}{c|}{0.193} & 52.10                                               & \multicolumn{1}{c|}{0.377} & 93.42                                               & \multicolumn{1}{c|}{0.189} & 64.55                                               \\
H-Sample Guidance           & \multicolumn{1}{c|}{0.113} & 51.46                                               & \multicolumn{1}{c|}{0.184} & 56.53                                               & \multicolumn{1}{c|}{0.118} & 57.63                                               \\
H-Distribution Guidance     & \multicolumn{1}{c|}{\textbf{0.049}} & \textbf{50.27}                                               & \multicolumn{1}{c|}{\textbf{0.113}} & \textbf{52.38}                                               & \multicolumn{1}{c|}{\textbf{0.014}} & \textbf{51.78}                                               \\ \midrule
Random sampling*            & \multicolumn{1}{l|}{0.307} & \multicolumn{1}{l|}{112.28}                         & \multicolumn{1}{l|}{0.463} & \multicolumn{1}{l|}{123.97}                         & \multicolumn{1}{l|}{0.276} & \multicolumn{1}{l}{117.83}                          \\
Magnet*                     & \multicolumn{1}{l|}{0.267} & \multicolumn{1}{l|}{91.15}                          & \multicolumn{1}{l|}{0.454} & \multicolumn{1}{l|}{97.05}                          & \multicolumn{1}{l|}{0.281} & \multicolumn{1}{l}{106.55}                          \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:single_attr}
\vspace{-7mm} 
\end{table} 


\noindent \textbf{Quantitative evaluation.} We evaluate our debiasing method for the single attribute case by generating balanced distributions of individual sensitive attributes - \textit{gender}, \textit{eyeglasses}, and \textit{race}, in Tab.~\ref{tab:single_attr}. For the scope of this paper, we consider all these attributes as binary, and hence expect a $1:1$ ratio of the sensitive attributes in the synthesized images (for e.g. $0.50$ fraction of males and $0.50$ fraction of females in case of gender). Specifically, we generate $10K$ images from each method per attribute and compute the metrics defined in Sec.~\ref{subsec:metrics}. The proposed guidance method outperforms all the methods in terms of visual quality as measured by FID and bias generation measured by FD. Sample guidance achieves comparable FID for \textit{gender}; however, higher FD indicates inferior debiasing. The tradeoff between FD and FID is discussed in detail in subsection \ref{subsec:ablate}. This supports our thesis that the distribution guidance provides enough flexibility during generation, resulting in high-quality outputs even with a high guidance scale.


\noindent \textbf{Multiple attributes.} Additionally, we apply our method for debiasing multiple attributes simultaneously in Tab.~\ref{tab:multi_attr}. Specifically, given two reference distributions $\mathbf{p^{a_1}_{ref}}$ and $\mathbf{p^{a_2}_{ref}}$, we add guidance from two pretrained attribute distribution predictors $g_{\psi_1}$ and $g_{\psi_2}$. For this experiment, we define both the reference distribution as uniform for each attribute ($50\%$-$50\%$ splits).
The generated results follow the reference distribution, resulting in a balanced generation across attributes.


\begin{table}[]
\vspace{-6mm} 
\caption{Evaluation of \textit{balanced} generation for multiple attribute}
\vspace{-3mm}
\begin{adjustbox}{width=0.45\textwidth,center}
\begin{tabular}{@{}l|cc|cc|cc@{}}
\toprule
                            & \multicolumn{2}{c|}{Gender + Race}                                               & \multicolumn{2}{c|}{Eyeglasses + Race}                                           & \multicolumn{2}{c}{Gender + Eyeglasses}                                          \\ \midrule
\multicolumn{1}{c|}{Metric} & \multicolumn{1}{c|}{FD $\downarrow$}    & \begin{tabular}[c]{@{}c@{}}FID $\downarrow$\\ \end{tabular} & \multicolumn{1}{c|}{FD $\downarrow$}    & \begin{tabular}[c]{@{}c@{}}FID $\downarrow$\\ \end{tabular} & \multicolumn{1}{c|}{FD $\downarrow$}    & \begin{tabular}[c]{@{}c@{}}FID $\downarrow$\\ \end{tabular} \\ \midrule
Random Sampling             & \multicolumn{1}{c|}{0.256} & 60.68                                               & \multicolumn{1}{c|}{0.292} & 89.14                                               & \multicolumn{1}{c|}{0.214} & 70.97                                               \\
Universal Guidance          & \multicolumn{1}{c|}{0.283} & 71.84                                               & \multicolumn{1}{c|}{0.264} & 91.54                                               & \multicolumn{1}{c|}{0.157} & 80.57                                               \\
H-Sample Guidance           & \multicolumn{1}{c|}{0.241} & 59.78                                               & \multicolumn{1}{c|}{0.135} & 67.87                                               & \multicolumn{1}{c|}{0.079} & 52.03                                               \\
H-Distribution Guidance     & \multicolumn{1}{c|}{\textbf{0.075}} & \textbf{49.91}                                               & \multicolumn{1}{c|}{\textbf{0.101}} & \textbf{57.46}                                               & \multicolumn{1}{c|}{\textbf{0.057}} & \textbf{47.45}                                               \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:multi_attr}
\vspace{-7mm}
\end{table}


\noindent \textbf{Comparison with MagNet}~\cite{humayun2021magnet}: MagNet is an unsupervised method enabling \textit{fair} sampling from a pretrained model. They propose a method for uniform sampling on the image manifold to generate under-represented groups equally. We generated results by MagNet sampling from a StyleGAN2~\cite{sg2} model trained on the FFHQ~\cite{ffhq} dataset from their official codebase. We compare our method with MagNet~\cite{humayun2021magnet} for the task of fair generation in Tab.~\ref{tab:single_attr}. We used MagNet to generate $10K$ samples and compute the FD score. As the base model for MagNet is StyleGAN2, we cannot compare FID directly with our DM debiased results. However, we can observe that MagNet achieves similar FD scores to its baseline model and is ineffective in debiasing the three sensitive attributes: gender, race, and eyeglasses. However, our distribution guidance significantly improves the FD metric from the baseline DM model. 

\noindent
\textbf{Qualitative evaluation.} We present qualitative results for attribute balancing with respect to \textit{gender} and \textit{eyeglasses} in Fig.~\ref{fig:single-debias}. We randomly sample $20$ starting noise and use individual guidance methods for debiasing. Without guidance, the DM mostly generates \textit{female} faces for the gender attribute. Sample guidance and universal guidance, although increasing the number of \textit{males}, collapses some images. On the other hand, Distribution guidance generates an almost equal number of males and females without affecting the generation quality. Moreover, the DM hardly generates images with \textit{eyeglasses} for sample and universal guidance and also without any guidance. Our method, on the contrary, leads to highly balanced generations.

\subsection{Generating Imbalanced Distributions} 
\vspace{-2mm}
We tested our distribution guidance for generating imbalanced attribute distribution by providing skewed $\mathbf{p^a_{ref}}$ - \textbf{i)} $0.20$ \textit{female} and $0.80$ \textit{male} \textbf{ii)} $0.10$ \textit{white race} and $0.90$ \textit{black race}. These two settings are extremely challenging given that \textit{male} and \textit{black race} are minority groups in the dataset. We present qualitative results for both the settings in Fig.\ref{fig:skew_generation}, where our distribution guidance is able to generate the defined distribution with majority \textit{males}. Note, we have binarized the race attribute as \textit{black} and \textit{whites} for simplicity, and hence in the generation \textit{brown race} is considered under \textit{black} category.
We report quantitative metrics in Tab.~\ref{tab:skew_bias_gen}, where the proposed method can achieve good FD scores with the same FID. 


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/cvpr24-debdiff-skew-fig9-gen.pdf}
    \vspace{-6mm}
    \caption{Generating imbalanced data with two non-uniform reference distribution - \textbf{i) 0.9B-0.1W}, \textbf{ii) 0.8M-0.2F.} \textcolor{Goldenrod} {Minority classes} are marked. Distribution guidance generates high-quality images and \textit{closely follows} the skewed reference distribution.}
    \vspace{-6mm}
    \label{fig:skew_generation} 
\end{figure}


\begin{table}[]
\caption{Distribution guidance for imbalanced generation}
\vspace{-2mm}
\begin{adjustbox}{width=0.40\textwidth,center}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{1}{c}{}                         & \multicolumn{2}{l}{\textbf{0.20F - 0.80M}}       & \multicolumn{2}{l}{\textbf{0.10W - 0.90B}}      \\ \midrule
\multicolumn{1}{c|}{Method}                  & \multicolumn{1}{c}{FD} & \multicolumn{1}{c|}{FID} & \multicolumn{1}{c}{FD} & \multicolumn{1}{c}{FID} \\ \midrule
\multicolumn{1}{c|}{Random Sampling}                  & \multicolumn{1}{c}{0.478} & \multicolumn{1}{c|}{72.26} & \multicolumn{1}{c}{0.734} & \multicolumn{1}{c}{77.63} \\ \midrule
\multicolumn{1}{c|}{H-Distribution Sampling}                  & \multicolumn{1}{c}{\textbf{0.168}} & \multicolumn{1}{c|}{\textbf{51.65}} & \multicolumn{1}{c}{\textbf{0.325}} & \multicolumn{1}{c}{\textbf{53.80}} \\ \midrule

%\multicolumn{1}{c|}{Random Sampling}         &  72.26                 & 0.478 \multicolumn{1}{c|}{} &    77.63  &      0.734                \\
% \multicolumn{1}{c|}{H-Distribution Guidance} &  51.65                 &  0.168 \multicolumn{1}{c|}{} &    53.80 &     0.325                       \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:skew_bias_gen}
\vspace{-7mm}
\end{table}

\subsection{Ablations}
\label{subsec:ablate}
\vspace{-2mm}
\textbf{Guidance Strength $\gamma$}. We ablate over guidance strength parameter $\gamma$ for both the distribution guidance and sample guidance in Fig.~\ref{fig:guidance_ablation}. Increasing $\gamma$ reduces the bias (better FD) at the cost of inferior image quality (increased FID). Guidance strength $1500$ achieved a good tradeoff between image quality and balancing attributes. Further, as compared to sample guidance, the distribution guidance achieves a better tradeoff for all the guidance strengths. 


\begin{figure}[h]
    \centering 
    \includegraphics[width=\linewidth]{figs/cvpr24-debdiff-ablation-fig8-guidance-strength.pdf}
    \caption{Ablation over guidance strength $\gamma$}
    \label{fig:guidance_ablation} 
\end{figure}


\noindent \textbf{Batch size.} As we approximate $\mathbf{p^a_{\theta}}$ with a an estimate $\mathbf{\hat{p}^a_\theta}$ over a batch of size $N$, we ablate over different values of $N$ in Tab.~\ref{tab:ablate_bs}. Intuitively, using a larger batch size yields a better estimate of $\mathbf{p^a_{\theta}}$.
We have found that the $N=100$ works best for all our experiments. 


\begin{table}[h]
\caption{Ablation over batch size for gender balancing.}
\vspace{-3mm}
\begin{adjustbox}{width=0.35\textwidth,center}
\begin{tabular}{@{}c|ccccc@{}}
\toprule
Batch size & 10    & 25    & 50    & 75    & 100   \\ \midrule
FD   $\downarrow$      & 0.062 & 0.059 & 0.049 & 0.059 & 0.046 \\
FID   $\downarrow$     & 50.54 & 51.51 & 50.86 & 50.98 & 51.64 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:ablate_bs}
\vspace{-6mm}
\end{table}

% \noindent \textbf{Number of training examples.} Our attribute classifiers are implemented as a linear head over the \textit{h-space} features; Hence, it does not require fewer training examples than the image-based classifiers. We ablate with a different number of training examples in Tab.{}. Observe that the classifiers trained with fewer examples achieve comparable accuracy. In practice, we have observed that $2K$ examples are enough to learn classifiers to perform distribution guidance.  

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/cvpr24-fig6-stablediff-gender.pdf}
    \vspace{-8mm}
    \caption{Debiasing results on stable diffusion for gender attribute. The proposed distribution guidance can balance the \textit{gender} attributes in the neutral prompt and generalizes well to prompts involving other professions \eg. \textit{firefighter}, \textit{doctor}.}
    \label{fig:stable-diff}
    \vspace{-4mm} 
\end{figure*}

\subsection{Experiments on Stable Diffusion}
\label{subsec:sd_exp}
\vspace{-2mm}
We implemented our distribution guidance technique for debiasing a text-to-image generation model, Stable Diffusion (SD) v1.5~\cite{ldm} concerning the \textit{gender} attribute in this subsection. First, we generate a dataset $\mathcal{D}$, of $10K$ images from SD, with prompts \textit{`a photo of a male'} and \textit{`a photo of a female'} to generate a labeled dataset for training h-space classifiers. If we use the same CelebA-HQ dataset to train the \textit{h-space} classifier, the guidance is ineffective due to a significant domain shift from the SD generations. Next, we obtain the corresponding labeled dataset $\mathcal{D}^h_{clf}$ in the \textit{h-space} and train a \textit{gender} classifier in the h-space. We used the trained classifier for distribution guidance following Sec.~\ref{subsec:guide_h_space} to generate images with balanced \textit{gender}.  

It is observed that SD increases the gender bias when queried to generate certain professions (\eg male and doctor)~\cite{zhang2023iti}. To this end, we implement our distribution guidance along the prompts \textit{`a photo of a doctor'} and \textit{`a photo of a firefighter'} to evaluate the effectiveness in this challenging setting. The qualitative results are shown in Fig.\ref{fig:stable-diff}, and the quantitative results are reported in Tab.~\ref{tab:sd_metrics}. 

\noindent \textbf{Baselines.} We compare our method with the following methods. (1) Random sampling from Stable Diffusion ~\cite{ldm} without any modifications. (2) ITI-Gen ~\cite{zhang2023iti} that learns a set of prompt embeddings for each class of the attribute given a reference set, and uses these embeddings to balance the generations. (3) Fair Diffusion ~\cite{friedrich2023fairdiffusion} that uses a lookup tabel to recognize the biased concept from the text input and adds scaled attribute expressions to the prompt.
% We can observe, as compared to the \textbf{baseline} (random generation without guidance), our method generates \textit{fairer} gender distribution with both neutral prompts and prompts mentioning professions (\textit{\eg. `a photo of a firefighter'}). Additional results on text-to-image models are present in supp. material.


\begin{table}[]
\caption{Balancing \textit{gender} on Stable Diffusion~\cite{ldm} model.}
\vspace{-3mm}
\begin{adjustbox}{width=0.45\textwidth, center}
\begin{tabular}{@{}l|cc|cc|cc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{2}{c|}{Gender}        & \multicolumn{2}{c|}{Doctor}        & \multicolumn{2}{c}{Firefighter}    \\ \cmidrule(l){2-7} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{FD $\downarrow$}    & FID $\downarrow$   & \multicolumn{1}{c|}{FD $\downarrow$}    & FID $\downarrow$  & \multicolumn{1}{c|}{FD $\downarrow$}    & FID $\downarrow$  \\ \midrule
Random Sampling                              & \multicolumn{1}{c|}{0.317} & 72.37 & \multicolumn{1}{c|}{0.355} & 70.11 & \multicolumn{1}{c|}{0.235} & 71.86 \\
ITI-Gen ~\cite{zhang2023iti}                               & \multicolumn{1}{c|}{0.049} &  & \multicolumn{1}{c|}{0.072} &  & \multicolumn{1}{c|}{0.184} &  \\
Fair Diffusion ~\cite{friedrich2023fairdiffusion}                            & \multicolumn{1}{c|}{0.227} &  & \multicolumn{1}{c|}{0.035} &  & \multicolumn{1}{c|}{0.036} &  \\
H-Sample Guidance                            & \multicolumn{1}{c|}{0.026} & 70.96 & \multicolumn{1}{c|}{0.021} & 68.43 & \multicolumn{1}{c|}{0.097} & 70.42 \\
H-Distribution Guidance                      & \multicolumn{1}{c|}{\textbf{0.024}} & \textbf{70.69} & \multicolumn{1}{c|}{\textbf{0.015}} & \textbf{67.36} & \multicolumn{1}{c|}{\textbf{0.093}} & \textbf{69.41} \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:sd_metrics}
\vspace{-6mm} 
\end{table} 



% \subsection{Debiasing attribute classifier}
% \vspace{-2mm}
% We explore an important downstream application of our proposed approach in debiasing an attribute classifier by augmenting the training dataset with samples from minority groups. Specifically, we trained a race classifier (labels obtained from $\mathcal{C}_\mathcal{A}$) on the CelebA-HQ~\cite{celebA-hq} dataset. The race classifier was an ImageNet~\cite{deng2009imagenet} pretrained ResNet-18~\cite{he2016deep} encoder, followed by 2 MLP layers and a classifier. We manually injected spurious correlations between the \textit{Race} and \textit{Gender} by oversampling the \textit{White}s and undersampling the \textit{Black}s in the training dataset. The biased dataset consisted of $10k$ samples of white people and $1k$ black people, both gender-balanced within a race class. Consequently, the model performed poorly on the minority groups (i.e., black males and black females) due to under-representation. Next, we augmented (balanced) the training data by generating samples whose distribution was inversely proportional to the group counts to increase images of underrepresented groups from our distribution guidance. This added 9k gender-balanced images of only \textit{Black} race. The trained classifier on this group-balanced data performs significantly better in the group-wise accuracy (Tab. \ref{tab:downstream_classifier}). This shows a potential application in generating `attribute' balanced datasets to train models for other downstream tasks. 

\subsection{Class-imbalance in attribute classification}
\vspace{-2mm}
We explore an important downstream application of our proposed approach in balancing minority classes by augmenting the under-represented classes with generated data. Specifically, we train a race classifier (labels obtained from $\mathcal{C}_\mathcal{A}$) on the CelebA-HQ~\cite{celebA-hq} dataset. The race classifier is an ImageNet~\cite{deng2009imagenet}-pretrained ResNet-18~\cite{he2016deep} encoder, followed by 2 MLP layers and a classifier. We manually oversample the \textit{White}s and undersample the \textit{Black}s in the training dataset such that the imbalanced dataset consists of $10k$ samples of white people and $1k$ black people (we keep the genders balanced within a race class). Consequently, the model performs poorly on the minority class (i.e., \textit{Black}) due to under-representation. Next, we augment (class-balanced) the training data by generating samples whose distribution is inversely proportional to the class counts in the training set to increase images of minority classes using our distribution guidance approach. This adds 9k images of only \textit{Black} race, and the classifier trained on this balanced data performs significantly better (Tab. \ref{tab:downstream_classifier}). Even when gender is balanced in both the classes, we observe a significant disparity in the accuracies for Male and Female \textit{Black} samples in the vanilla classifier. However, our proposed method helps reduce the accuracy gap between Black males and Black females. This shows a potential application in generating 'class' balanced datasets to train models for other downstream tasks, which can also mitigate bias.

\begin{table}[]
\caption{Group-wise accuracies of identical classifiers trained on existing and generated(balanced) data}
\vspace{-3mm}
\begin{adjustbox}{width=0.45\textwidth,center}
\begin{tabular}{@{}l|c|c|c|c@{}}
\toprule
                    & Black female & White female & Black male & White male \\ \midrule
Vanilla classifier  & 75.76        & 98.96      & 70.29        & 99.93      \\
Balanced classifier & 91.04        & 97.33      & 90.72        & 97.68      \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:downstream_classifier}
\vspace{-6mm}
\end{table}

\vspace{-1mm}
\section{Discussion.}
\vspace{-2mm} 

\textbf{Limitations.} 
Although our method performs guidance in the \textit{h-space}, which is efficient compared to the image space guidance, it still requires additional training of \textit{h-space} classifiers. Another limitation is reliance on accurate attribute classifiers to obtain labels for training \textit{h-space} classifiers. 

\noindent \textbf{Future works.} An important future work is extending distribution guidance beyond de-biasing for controlled generation and data augmentation. In the context of debiasing DMs, extending the proposed approach without needing an attribute classifier or labeled data. 

\section{Conclusion}
\vspace{-2mm}
In this work, we aim to mitigate biases from pretrained diffusion models without retraining - given only a desired reference attribute distribution.
% We propose a technique to mitigate the biases from pretrained diffusion models, given a reference attribute distribution. 
We propose a novel approach leveraging \textit{distribution guidance} that jointly guides a batch of images to follow the reference attribute distribution. The proposed method is effective and results in both high-quality and \textit{fair} generations across multiple attributes and outperforms sample guidance strategies based on conditioning each sample individually. Extensive experiments demonstrate the effectiveness of our method in balancing both single and multiple attributes on unconditional DMs and conditional text-to-image diffusion models. We believe such a setting of debiasing without retraining is practical, especially in today's era of large-scale generative models.  

% Finally, we showed the generated data can be used to augment the data for under-represented groups, resulting in fair attribute classifiers.
